Towards Dark Jargon Interpretation in Underground Forums

Dark jargons are benign-looking words that have hidden, sinister meanings and are used by participants of underground forums for illicit behavior. For example, the dark term "rat" is often used in lieu of "Remote Access Trojan". In this work we present a novel method towards automatically identifying and interpreting dark jargons. We formalize the problem as a mapping from dark words to "clean" words with no hidden meaning. Our method makes use of interpretable representations of dark and clean words in the form of probability distributions over a shared vocabulary. In our experiments we show our method to be effective in terms of dark jargon identification, as it outperforms another related method on simulated data. Using manual evaluation, we show that our method is able to detect dark jargons in a real-world underground forum dataset.

==> src/2_related_work.tex <==
\section{Related Work}

Recently, there has been substantial research interest in the intersection of Cybersecurity, Information Retrieval~\cite{husari2017ttpdrill,husari2018using,khandpur2017crowdsourcing,liao2016acing,liao2016seeking,mittal2016cybertwitter,mulwad2011extracting,tsai2007detecting}, and Natural Language Processing~\cite{lim2017malwaretextdb,seyler2018identifying,zhou2018automatic,zhu2016featuresmith,zhu2018chainsmith}. 
Two works are directly related to our problem setup: Yang et al.~\cite{yang2017learn} proposes a method to detect dark jargon by utilizing a search engine. The authors scrape data from pages that tend to contain dark terms, filter out key words and use the search engine's similar search function to discover new dark words. In contrast, our method does not rely on external resources, such as search engines.
In Yuan et al.~\cite{Yuan2018ReadingTC}, the authors leverage the context of a word as a representation for the word's meaning. The intuition is that dark words in dark forums appear in drastically different contexts compared to reputable online corpora (e.g., Wikipedia). 
Even though the idea of context representation is similar, our method provides more interpretable meaning representations.
Another shortcoming of previous approaches is that the actual meaning of the identified dark jargon is unknown. 
In Yuan et al.~\cite{Yuan2018ReadingTC} dark words are categorized into five general classes. For example, ``blueberry'' is categorized as ``drug'' and not as ``marijuana'', which would be more beneficial for interpretation. Our framework is more expressive since it allows dark terms to be mapped to any word in the clean corpus, where the meaning is known.


